Frame-wise and overlap-robust speaker embeddings for meeting diarization

Using a Teacher-Student training approach we developed a speaker embedding extraction system that outputs embeddings at frame rate. Given this high temporal resolution and the fact that the student produces sensible speaker embeddings even for segments with speech overlap, the frame-wise embeddings serve as an appropriate representation of the input speech signal for an end-to-end neural meeting diarization (EEND) system. We show in experiments that this representation helps mitigate a well-known problem of EEND systems: when increasing the number of speakers the diarization performance drop is significantly reduced. We also introduce block-wise processing to be able to diarize arbitrarily long meetings.

==> symbols.tex <==
%% This file contains math symbols used in equations
% Use the \defm command to define a symbol

%% TODO: remove color at the end

% Give math macros a color so that it's easier to spot when variables are typed without macro.
% The macro can be exchanged for the second line for the final color-free version
%\newcommand\defm[2]{\expandafter\newcommand{#1}{\ensuremath{{\textcolor{purple}{#2}}}}}
\newcommand\defm[2]{\expandafter\newcommand{#1}{\ensuremath{#2}}} % variant without color (final)

%% Operators and other math macros
\newcommand{\matr}[1]{\ensuremath{\boldsymbol{\mathbf{#1}}}}
\newcommand{\vect}[1]{\ensuremath{\boldsymbol{\mathbf{#1}}}}
\newcommand*{\tran}{^{\mkern-1.5mu\mathsf{T}}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\sqnorm}[1]{\norm{#1}^2}
\newcommand{\loss}[1]{\Loss^{\text{(#1)}}}
\defm\conv{*}

%% Symbols
\defm\mix{y}
\defm\image{x}
\defm\source{s}
\defm\rir{h}
\defm\noise{\nu}
\defm\offset{\tau}
\defm\timeframe{t}
\defm\utt{n}
\defm\nutt{N}
\defm\scale{\alpha}
\defm\nspk{K}
\defm\spk{k}
\defm\activity{\pi}
\defm\estactivity{\hat{\activity}}
\defm\prob{p}

==> tikz_style.tex <==
\usepackage{tikz}
\usepackage{pgfplots}
\pgfplotsset{compat=1.16}
\usepgfplotslibrary{groupplots}
\usetikzlibrary{positioning,arrows,matrix,fit,calc,patterns,chains,scopes,shapes.multipart,decorations,decorations.markings,backgrounds}
% \usetikzlibrary{patterns}

% Colormap "muted"
\definecolor{palette-1}{HTML}{001C7F}    
\definecolor{palette-2}{HTML}{B1400D}    
\definecolor{palette-3}{HTML}{12711C}    
\definecolor{palette-4}{HTML}{8C0800}    
\definecolor{palette-5}{HTML}{591E71}    
\definecolor{palette-6}{HTML}{592F0D}    
\definecolor{palette-7}{HTML}{A23582}    
\definecolor{palette-8}{HTML}{3C3C3C}    
\definecolor{palette-9}{HTML}{B8850A}    
\definecolor{palette-10}{HTML}{006374}      

\tikzset{
    % Arrows
    line/.style={draw,black,thick,rounded corners=1mm,line cap=round},
    noshortarrow/.style={line,->},
    arrow/.style={noshortarrow,shorten >=.3mm},
    doublearrow/.style={arrow,<->, shorten <=.3mm},
    % Simple box
    box/.style={draw,black,minimum height=3em,text height=1.5ex,text depth=0.25ex,rounded corners=2,fill=white},
    nopadding/.style={minimum height=0,inner sep=1mm},
    % Primary box
    pbox/.style={box,fill=black!10},
    % Dashed background box
    backgroundbox/.style={inner xsep=3mm, inner ysep=1mm, draw, dashed, rounded corners,fill=orange!10},
    % This is a simple dot that can be used as a branch marker
    branch/.style={inner sep=0.3mm,circle,fill=black},
    % A circle that is supposed to contain a single operator like `node[operator] {$\times$};`
    operator/.style={draw,circle,black,rounded corners,inner sep=0,fill=white},
    % Fill patterns
    pattern1/.style={pattern=north west lines,pattern color=palette-1},
    pattern2/.style={pattern=north east lines,pattern color=palette-2},
    pattern3/.style={pattern=crosshatch,pattern color=palette-3},
    % Utterance boxes
    utt/.style={box,minimum height=1mm,inner sep=0,rounded corners=0.5,text=white,font=\footnotesize\sffamily},
    utt1/.style={utt,fill=palette-1, minimum width=1.5cm},
    utt2/.style={utt,fill=palette-2, minimum width=1cm},
    utt3/.style={utt,fill=palette-3, minimum width=1cm},
    utt4/.style={utt,fill=palette-4, minimum width=1cm},
    overlap/.style={fill=yellow,opacity=0.5},
    uttbox/.style={fill=black!15,draw=none,inner xsep=0,rounded corners=3},
}
